TraPHic: Trajectory Prediction in Dense and Heterogeneous Traffic Using Weighted Interactions

We present a new algorithm for predicting the near-term trajectories of road-agents in dense traffic videos. Our approach is designed for heterogeneous traffic, where the road-agents may correspond to buses, cars, scooters, bicycles, or pedestrians. We model the interactions between different road-agents using a novel LSTM-CNN hybrid network for trajectory prediction. In particular, we take into account heterogeneous interactions that implicitly accounts for the varying shapes, dynamics, and behaviors of different road agents. In addition, we model horizon-based interactions which are used to implicitly model the driving behavior of each road-agent. We evaluate the performance of our prediction algorithm, TraPHic, on the standard datasets and also introduce a new dense, heterogeneous traffic dataset corresponding to urban Asian videos and agent trajectories. We outperform state-of-the-art methods on dense traffic datasets by 30%.

==> redundant.tex <==
There has been extensive progress in trajectory prediction using Recurrent Neural Networks (RNNs) such as Long Short-Term Memory (LSTM) methods \cite{social-lstm,graves}.

==> tables2.tex <==
% \begin{table*}[t]
%     \centering
%   \resizebox{0.2\textwidth}{!}{
%   \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
%   \hline
%     Dataset (\# classes) & Person &Car & Bike & Scooter & Bus & Truck & Cycle & Rickshaw &Animal\\
%     \hline
%     NGSIM(3) &9.5 &2 &0 &0 &0 &0 &0 &1.5 &0\\
%     KITTI (3) &13 &3 &0 &0 &0.5 &0 &0 &0  &0\\
%     Beijing (2) &13 &0 &0 &0 &0 &0.5 &0 &0 &0\\
%     \hline
%     \textbf{Our Dataset (8)} &\textbf{28.5} &\textbf{37} &\textbf{22} &\textbf{8} &\textbf{2} &\textbf{0.5} &\textbf{1.5} &\textbf{14.5} &\textbf{1}\\
%     \hline
%   \end{tabular}
%   }
%     \caption{Comparison of our dense and heterogeneous TRAF (TRAF11 and TRAf12) dataset with standard datasets in terms of heterogeneity and density.}
%     \label{dataset}
%     \vspace{-10pt}
% \end{table*}

